Total Variation Minimization in Compressed Sensing

This chapter gives an overview over recovery guarantees for total variation minimization in compressed sensing for different measurement scenarios. In addition to summarizing the results in the area, we illustrate why an approach that is common for synthesis sparse signals fails and different techniques are necessary. Lastly, we discuss a generalizations of recent results for Gaussian measurements to the subgaussian case.

==> Revised ArXiv/FourierData.tex <==
%Poon
\subsection{Recovery from subsampled Fourier measurements}
Fourier measurements are widely used in many applications.
Especially in medical applications as parallel-beam tomography and magnetic resonance imaging it is desirable to reduce the number of samples to spare patients burden.
In Section \ref{suffcond}, this is a motivation for introducing algorithmic checks for unique solutions of \eqref{eq:ExactTV}. In this section, we consider a probabilistic approach where an incomplete measurement matrix $A\in\mathbb{C}^{m\times n}$ chosen from the discrete Fourier transform on $\mathbb{C}^N$ is considered.
Therefore we consider a subset $\Omega$ of the index set $\{-\lfloor n/2\rfloor+1,...,\lceil n/2\rceil\}$, where $\Omega$ consists of $m$ integers chosen uniformly at random and, additionally, $0\in\Omega$. 
Hence, we want to recover a signal, sparse in the gradient domain, with a measurement matrix $A = (e^{2\pi ikj/n})_{k\in\Omega,j\in[n]}$.
In \cite{crt2006robust} the optimal sampling cardinality for $s$-sparse signals in the gradient domain was given and enables to recover one-dimensional signals signals from $\mathcal{O}(k\log(n))$ Fourier samples.
It naturally extends to two dimensions.

\begin{theo}\cite{crt2006robust}
With probability exceeding $1-\eta$, a signal $z$, which is $k$-sparse in the gradient domain is the unique solution of \eqref{eq:ExactTV} if \[m\gtrsim k(\log(n)+\log(\eta^{-1})).\]
\end{theo}
As already discussed in the introduction, the proof of this result proceeds via  recovering the gradient and then using that the discrete gradient (with periodic boundary conditions) is injective. Due to the poor conditioning of the gradient, however, this injectivity results do not directly generalize to recovery guarantees for noisy measurements. For two (and more) dimensions, such results can be obtained via the techniques discussed in the previous subsection. 

These techniques, however, do not apply directly. Namely, the Fourier (measurement) basis is not incoherent to the Haar wavelet basis; in fact, the constant vector is contained in both, which makes them maximally coherent. As observed in \cite{pvw11}, this incoherence phenomenon only occurs for low frequencies, the high frequency Fourier basis vectors exhibit small inner products to the Haar wavelet basis. This can be taken into account using a {\em variable density} sampling scheme with sampling density that is larger for low frequencies and smaller for high frequencies. For such a sampling density, one can establish the restricted isometry for the corresponding randomly subsampled discrete Fourier matrix combined with the Haar wavelet transform with appropriately rescaled rows \cite{KW14}. This yields the following recovery guarantee.

\begin{theo}\cite{KW14}
	\label{thm1}
	Fix integers $N = 2^p, m,$ and $s$ such that $s\gtrsim \log(N)$ and 
	\begin{equation}
	\label{m:tv}
	m \gtrsim s \log^{3}(s)\log^5(N).
	\end{equation}
	Select $m$ frequencies $\{ (\omega_1^j, \omega_2^j ) \}_{j=1}^m \subset \{-N/2+1, \dots, N/2\}^2$ i.i.d. according to
	\begin{equation}
	\label{inverseD}
	\mathbb{P} \big[ (\omega_1^j, \omega_2^j) = (k_1, k_2) \big]  = C_N \min\left(C, \frac{1}{k_1^2 + k_2^2 }\right) =: \eta(k_1, k_2), \quad -N/2+1 \leq k_1, k_2 \leq N/2,
	\end{equation}
	where $C$ is an absolute constant and $C_N$ is chosen such that $\eta$ is a probability distribution. \\
	Consider the weight vector $\rho = (\rho_j)_{j=1}^m$ with $\rho_j = (1/\eta(\omega^j_1, \omega^j_2))^{1/2}$, and assume that the noise vector $\xi = (\xi_j)_{j=1}^m$ satisfies $\|\rho \hspace{.5mm} \circ \hspace{.5mm}  \xi\|_2\leq  \varepsilon \sqrt{m} $, for some $\epsilon>0$.  Then with probability exceeding $1 - N^{-C\log^3(s)}$, the following holds for all images $f \in \C^{N \times N}$:
	
	\noindent Given noisy partial Fourier measurements $y = {\cal F}_{\Omega}f + \xi$, the estimation
	\begin{equation}
	\label{TV}
	f^{\#} = \argmin_{g \in \C^{N \times N}} \| g \|_{TV}  \quad  \textrm{such that}  \quad \|\rho\circ( {\cal F}_{\Omega} g - y) \|_2   \leq \varepsilon\sqrt{m},
	\end{equation}
	where $\circ$ denotes the Hadamard product, approximates $f$ up to the noise level and best $s$-term approximation error of  its gradient:
	\begin{equation}
	\label{stable3}
	\| f -f^{\#} \|_2 \lesssim  \frac{ \| \nabla f -  (\nabla f)_s \|_1}{\sqrt{s}}+ \varepsilon.
	\end{equation}
\end{theo}


A similar optimality result is given in \cite{poon2013roleoftv}, also for noisy data  and inexact sparsity. In contrast to the previous result, this result includes the one-dimensional case.
The key to obtaining such a result is showing that the stable gradient recover implies the stable signal recovery, i.e.,
\begin{align}
\|z\|_2\lesssim\gamma+\Vert z\Vert_{TV}\mbox{ with }\|Az\|_2\le\gamma.\label{eq:sobolevemb}
\end{align}
Again the sampling distribution is chosen as a combination of the uniform distribution and a decaying distribution.
The main idea is to use this sampling to establish \eqref{eq:sobolevemb} via the RIP.
We skip technicalities for achieving the optimality in the following theorem and refer to the original article for more details. 

\begin{theo}\cite{poon2013roleoftv}
Let $z\in\mathbb{C}^n$ be fixed and $x$ be a minimizer of \eqref{eq:NoisyTV} with $\eps = \sqrt{m}\delta$ for some $\delta>0$, $m\gtrsim k\log(n)(1+\log(\eta^{-1}))$, and an appropriate sampling distribution.
Then with probability exceeding $1-\eta$, it holds that
\[\|\nabla z-\nabla x\|_2\lesssim\left(\delta\sqrt{k}+C_1\frac{\|P\nabla z\|_1}{\sqrt{k}}\right), \frac{\|z-x\|_2}{\sqrt{n}}\lesssim C_2\left(\frac{\delta}{\sqrt{s}}+C_1\frac{\|P\nabla z\|_1}k\right),\]
where $P$ is the orthogonal projection onto a $k$-dimensional subspace, 
\[C_1 = \log(k)\log^{1/2}(m)\mbox{, and }C_2 = \log^2(k)\log(n)\log(m).\] 
\end{theo}

In the two-dimensional setting the result changes to 
\[\|\nabla z-\nabla x\|_2\lesssim\left(\delta\sqrt{k}+C_3\frac{\|P\nabla z\|_1}{\sqrt{k}}\right), \|z-x\|_2\lesssim C_2\left(\delta+C_3\frac{\|P\nabla z\|_1}k\right),\]
with remaining $C_2$ and
\[C_3 = \log(k)\log(n^2/k)\log^{1/2}(n)\log^{1/2}(m).\]
These results are optimal since the best error one can archive \cite{needell2013stablereconsttv} is $\|z-x\|_2\lesssim \|P\nabla z\|_1k^{-1/2}$.

The optimality in the latter theorems is achieved by considering a combination of uniform random samling and variable density sampling.
Uniform sampling on its own can achieve robust and stable recovery.
However, the following theorem shows that the signal error is no longer optimal but the bound on the gradient error is still optimal up to log factors.
Here \eqref{eq:sobolevemb} is obtained by using the Poincar\'e inequality.

\begin{theo}\cite{poon2013roleoftv}
Let $z\in\mathbb{C}^n$ be fix and $x$ be a minimizer of \eqref{eq:NoisyTV} with $\eps = \sqrt{m}\delta$ for some $\delta>0$ and $m\gtrsim k\log(n)(1+\log(\eta^{-1}))$ with random uniform sampling.
Then with probability exceeding $1-\eta$, it holds that
\[\|\nabla z-\nabla x\|_2\lesssim\left(\delta\sqrt{k}+C\frac{\|P\nabla z\|_1}{\sqrt{k}}\right), \frac{\|z-x\|_2}{\sqrt{n}}\lesssim(\delta\sqrt{s}+C\|P\nabla z\|_1),\]
where $P$ is the orthogonal projection onto a $k$-dimensional subspace and $C = \log(k)\log^{1/2}(m)$.
\end{theo}
%
%Alternatively, one can also follow the lines of the previous subsection, using incoherence properties of the Fourier measurement basis with respect to Haar Wavelets. However, these two bases are not incoherent in the sense of ???. This concerns, however, only few vectors of the measurement basis, more specifically, those corresponding to low frequencies. ...

==> Revised ArXiv/RecovCondNoNoise.tex <==
% Section Recovery Conditions

\subsection{Sufficient Recovery Conditions}\label{suffcond}

Given linear measurements $Ax = y$ for an arbitrary $A\in \R^{m\times n}$ and a signal $x$ with $\|\nabla x\|_0 \le s$,
a natural way to recover $x$ is by solving
\begin{equation}\label{eq:ExactTV}\text{minimize } \| \nabla z\|_1\,\,\text{such that } Az=y.\end{equation}
For $I\subset[n]$ we denote $A_I$ as the columns of $A$ indexed by $I$, and for a consecutive notation we denote $\identitymatrix_{I}^T\nabla$ as the rows of $\nabla$ indexed by $I$ and $\identitymatrix$ as the identity matrix.
The following results can also be easily applied to \emph{analysis $\ell_1$-minimization}, where any arbitrary matrix $D\in\R^{p\times n}$ replaces $\nabla$ in \eqref{eq:ExactTV}, as well as to any real Hilbert space setting \cite{kruschel2015phd}.

In many applications it is important to verify whether there is exactly one solution of~\eqref{eq:ExactTV}.
Since $\nabla$ is not injective here, we cannot easily use the well-known recovery results in compressed sensing \cite{foucart2013mathematical} for the matrix $A\nabla^\dagger$.
However, a necessary conditon can be given since $x$ can only satisfy $Ax = y$ and $(\nabla x)_{I^c} = 0$ if
\begin{align*}
\mbox{ker}(\identitymatrix_{I^c}^T\nabla)\cap\mbox{ker}(A) = \{0\}.
\end{align*}
If $\nabla$ is replaced by the identity, this is equivalent to $A_I$ being injective.
Since this injectivity condition is unavoidable, we assume for the rest of this section that it is satisfied.

The paper~\cite{nam2013cosparse} provides sufficient and necessary conditons for uniform recovery via \eqref{eq:ExactTV}.
The conditions rely on the null space of the measurements and are hard to verify similar to the classical compressed sensing setup~\cite{tillmann2014complexity}.
The following result is a corollary of these conditions. It no longer provides a necessary condition, but is more manageable.
%
%If $\nabla$ is replaced by the identity, this is similar to the well-known \emph{null space property} \cite{donohohuo2001NSP}. 
%
\begin{coro}\cite{nam2013cosparse}\label{corr:TVNSP}
For all $x\in\R^n$ with $s:= \Vert \nabla x\Vert_0$, the solution of \eqref{eq:ExactTV} with $y=Ax$ is unique and equal to $x$ if for all $I\subset[n]$ with $|I|\le s$ it holds that
\[
\forall w\in\mathrm{ker}(A)\backslash\{0\}\colon\,\,
\|(\nabla w)_I\|_1 < \|(\nabla w)_{I^c}\|_1.
\]
\end{coro}
%
%A common strategy to tackle this uniform recovery condition will be considered in the subsequent sections by assuming random measurements of different kind.\\
To consider measurements for specific applications, where it is difficult to prove whether uniform recovery is guaranteed, one can empirically examine whether specific elements $x$ solve \eqref{eq:ExactTV} uniquely.
For computed tomography measurements, a \emph{Monte Carlo Experiment} is considered in \cite{Jorgensen2015uniquenessconditions} to approximate the fraction of all gradient $s$-sparse vectors to uniquely solve \eqref{eq:ExactTV}.
%By repeatedly checking different $x$ with $\Vert \nabla x\Vert_0=s$, for being a unique solution of \eqref{eq:ExactTV}, one can approximate among all gradient $s$-sparse vectors the fraction of those who can uniquely be recovered via TV minimization.  
%Such a \emph{Monte Carlo Experiment} is done in \cite{Jorgensen2015uniquenessconditions} where the TV-minimization is applied to computed tomography measurements.
%Here, different images $X\in\R^{n\times n}$ with gradient sparsity $s$ were constructed via a random model and tested whether they are unique solutions of \eqref{eq:ExactTV}.
The results prompt that there is a sharp transition between the case that every vector with a certain gradient sparsity is uniquely recoverable  and the case that TV-minimization will find a different solution than the desired vector. %\todo{unclear formulation -- Better?}
This behavior empirically agrees with the phase transition in the classical compressed sensing setup with Gaussian measurements \cite{donoho2004phasetransition}.
%The idea is that the non-deterministic construction simulates a random sampling of $s$-gradient-sparse images and since we choose a lot of these images by random, we can approximate the ratio of images being unique solutions and being no unique solution.

To efficiently check whether many specific vectors $x$ can be uniquely recovered via \eqref{eq:ExactTV}, one needs to establish characteristics of $x$ which must be easily verifiable.
Such a non-uniform recovery condition is given in the following theorem.

\begin{theo}\label{th:weakuniquenesscond}\cite{Jorgensen2015uniquenessconditions}
It holds that $x\in\R^n$ is a unique solution of \eqref{eq:ExactTV} if and only if there exists $w\in\R^m$ and $v\in\R^{n-1}$ such that
\begin{align}
\nabla^Tv = A^Tw, v_I = \mbox{sign}(\nabla x)_I, \Vert v_{I^c}\Vert_\infty < 1.\label{eq:uniquenesscondition}
\end{align}
\end{theo}
The basic idea of the proof is to use the optimality condition for convex optimization problems \cite{Rockafellar1972convex}.
Equivalent formulations of the latter theorem can be found in \cite{zhang2016uniquenessconditions,Kabanava2015uniquenessconditions} where the problem is considered from a geometric perspective.
However, verifying the conditions in Theorem \ref{th:weakuniquenesscond} still requires solving a linear program where an optimal $v$ for \eqref{eq:uniquenesscondition} needs to be found.
%\[
% \text{minimize } \Vert v\Vert_{\infty} \text{ such that } v_I = \mbox{sign}(\nabla x)_I, \nabla^T v\in\mbox{rg}(A^T).
%\]
In classical compressed sensing, the \emph{Fuchs Condition} \cite{fuchs2004condition} is known as a weaker result as it suggests a particular $w$ in \eqref{eq:uniquenesscondition} and avoids solving the consequential linear program.
The following result generalizes this result to general analysis $\ell_1$-minimization.

\begin{coro}
If $x\in\R^n$ satisfies
\[\|(\identitymatrix_{I^c}^T\nabla(\nabla^T\identitymatrix_{I^c}\identitymatrix_{I^c}^T\nabla+A^TA)^{-1}\nabla\mbox{sign}(\nabla x))_I\|_\infty < 1\]
then $x$ is the unique solution of \eqref{eq:ExactTV}.
\end{coro}



==> Revised ArXiv/RecoverySubgauss.tex <==
\section{TV-recovery from subgaussian measurements in 1D}\label{sec:RecoverySubgauss}

In this section, we will apply the geometric viewpoint discussed in~\cite{vershynin2014estimation} to the problem, which will eventually allow us to show the TV recovery results for noisy subgaussian measurements mentioned in Section~\ref{sec:RecoveryGauss}.

As in the original proof of the 1D recovery guarantees for Gaussian measurements \cite{cai2015guarantees}, the {\em Gaussian mean width} will play an important role in our considerations.
{\defi The (Gaussian) mean width of a bounded subset $K$ of $\R^n$ is defined as \[w(K) := \Ex \sup_{x\in K-K}\ip{g}{x},\]
	where $g\in\R^n$ is a vector of i.i.d. $\Ncal(0,1)$ random variables.
}
 
In \cite{cai2015guarantees}, the mean width appears in the context of the {\em Gordon's escape through the mesh} approach \cite{gordon1988milman} (see Section~\ref{sec:ExactRecov} below), but as we will see, it will also be a crucial ingredient in applying the Mendelson small ball method \cite{koltchinskii2015bounding, mendelson2014learning}.

The mean width has some nice (and important) properties, it is for example invariant under taking the convex hull, i.e.,
\[w(\ch(K))  = w(K).\]
Furthermore, it is also invariant under translations of $K$, as $(K-x_0) - (K-x_0) = K-K$.  Due to the rotational invariance of Gaussian random variables, that is $Ug\sim g$, we also have that $w(UK) = w(K)$.
Also, it satisfies the inequalities 
\[w(K) = \Ex \sup_{x\in K-K}\ip{g}{x}\leq 2\Ex\sup_{x\in K}\ip{g}{x}\leq 2\Ex\sup_{x\in K}|\ip{g}{x}|,\]
which are equalities if $K$ is symmetric about $0$, because then $K=-K$ and hence $K-K=2K$.

\subsection{$M^*$ bounds and recovery}
%One definition that will turn out to be extremely useful is the notion of \emph{mean width}.
In order to highlight the importance of the Gaussian mean width in signal recovery, we present some arguments from \cite{vershynin2014estimation}.
Thus in this section we present a classical result, the $M^*$ bound, which connects the mean width to recovery problems, cf.~\cite{vershynin2014estimation}. 
Namely, recall that due to rotational invariance, the kernel of a Gaussian random matrix $A\in\R^{m\times n}$ is a random subspace distributed according to the uniform distribution (the Haar measure) on the Grassmannian 

\[G_{n,n-m}:=\{V\leq \R^n\colon \dim(V) = n-m\}.\]

Consequently, the set of all vectors that yield the same measurements directly correspond to such a random subspace.

 The average size of the intersection of this subspace with a set reflecting the minimization objective now gives us an average bound on the worst case error.

{\theo[$M^*$ bound, Theorem~3.12 in \cite{vershynin2014estimation}]\label{theo:MStarBound} Let $K$ be a bounded subset of $\R^n$ and $E$ be a random subspace of $\R^n$ of drawn from the Grassmanian $G_{n,n-m}$ according to the Haar measure. Then
	\begin{equation}\label{M*bound}
	\Ex\, \diam(K\cap E) \leq C \frac{w(K)}{\sqrt{m}},
	\end{equation}
where $C$ is absolute constant.	
}



Given the $M^*$-bound it is now straightforward to derive bounds on reconstructions from linear observations. We first look at feasibility programs - which in turn can be used to obtain recovery results for optimization problems.
For that, let $K\subset \R^n$ be bounded and $x\in K$ be the vector we seek to reconstruct from measurements $Ax = y$ with a Gaussian matrix $A\in\R^{m\times n}$.

{\coro\label{theo:feasibility}\cite{mendelson2007reconstruction} Choose $\hat x\in \R^n$, such that 
	\[\hat x \in K\,\text{ and } A\hat x = y,\]
	then one has, for an absolute constant $C'$,
	\[\Ex \sup_{x\in K}\Vert \hat x - x\Vert_2 \leq C' \frac{w(K)}{\sqrt{m}}.\]
}

This corollary directly follows by choosing $C'=2C$, observing that $\hat x - x\in K-K$, and that the side constraint enforces $A(\hat x - x) = 0$.

Via a standard construction in functional analysis, the so called \emph{Minkowski functional}, one can now cast an optimization problem as a feasiblity program so that Corollary~\ref{theo:feasibility} applies.

{\defi The Minkowski functional of a bounded, symmetric set $K\subset \R^n$ is given by 
	\[\Vert\cdot\Vert_K\colon \R^n \to \R\colon x\mapsto \inf\{t>0\colon x\in tK\}.\]
}

So the Minkowski functional tells us, how much we have to 'inflate' our given set $K$ in order to capture the vector $x$. Clearly, from the definition we have that if $K$ is closed
\[K = \{x\colon \Vert x\Vert_K\leq 1\}.\]
If a convex set $K$ is closed and symmetric, then $\Vert\cdot\Vert_K$ defines a norm on $\R^n$.

Recall that a set $K$ is star shaped, if there exists a point $x_0\in K$, which satisfies that for all $x\in K$ we have $\{tx_0+(1-t)x\colon t\in[0,1]\}\subset K$.
It is easy to see that convex sets are star shaped, but for example unions of subspaces are not convex, but star shaped.

For bounded, star shaped $K$, the notion of $\Vert \cdot\Vert_K$ now allows to establish a direct correspondence between norm minimization problems and feasibility problems. With this observation, Corollary~\ref{theo:feasibility} translates to the following result.

{\coro\label{theo:opti} For $K$ bounded, symmetric and star-shaped, let $x\in K$ and $y=Ax$. Choose $\hat x\in \R^n$, such that it solves
	\[\min\Vert z\Vert_K \,\text{ with } Az = y,\]
	then
	\[\Ex \sup_{x\in K}\Vert \hat x - x\Vert_2 \leq C' \frac{w(K)}{\sqrt{m}}.\]
}

Here $\hat x\in K$ is due to the fact that the minimum satisfies $\Vert \hat x\Vert_K \leq \Vert x \Vert_K\leq 1$, as $x\in K$ by assumption. 

This result directly relates recovery guarantees to the mean width, it thus remains to calculate the mean width for the sets under consideration. In the following subsections, we will discuss two cases. The first one directly corresponds to the desired signal model, namely gradient sparse vectors. These considerations are mainly of theoretical interest, as the associated minimization problem closely relates to support size minimization, which is known to be NP hard in general. The second case considers the TV minimization problem introduced above, which then also yields guarantees for the (larger) set of vectors with bounded total variation.

Note, however, that the $M^*$-bound only gives a bound for the expected error. We can relate this result to a statement about tail probabilities using Markov's inequality, namely \[\Prob(\sup_{x\in K} \|x-\hat x\|_2>t)\leq t^{-1}\Ex \sup_{x\in K} \|x-\hat x\|_2\leq C'\frac{w(K)}{t\sqrt{m}}.\]

In the next section we compute the mean width for the set of gradient sparse vectors, that is we now specify the set $K$ in Corollary~\ref{theo:feasibility} to be the set of all vectors with energy bounded by one that only have a small number of jumps.


\subsection{The mean width of gradient sparse vectors in 1d}\label{sec:GradSparse}

Here~\cite{plan2013robust} served as an inspiration, as the computation is very similar for the set of sparse vectors.

{\defi The jump support of a vector $x$ is given via
	\[\tvsupp(x):= \{i\in[n-1]\colon x_{i+1}-x_i\neq 0\}.\]
}
The jump support captures the positions, in which a vector $x$ changes its values. With this, we now define the set 
\[K_0^s:= \{x\in\R^n\colon\Vert x\Vert_2\leq 1, |\tvsupp(x)|\leq s\}.\]
The set $K_0^s$ consists of all $s$-gradient sparse vectors, which have $2$-norm smaller than one. We will now calculate the mean width of $K_0^s$ in order to apply Corrolary~\ref{theo:feasibility} or~\ref{theo:opti}.

Note that we can decompose the set $K_0^s$ into smaller sets $K_J\cap B_2^n$ with $K_J=\{x\colon \tvsupp(x)\subset J\}$, $|J| = s$ and $B_2^n=\{x\in \R^n\colon \Vert x\Vert_2\leq 1\}$. As we can't add any jumps within the set $K_J$, it is a subspace of $\R^n$. We can even quite easily find an orthonormal basis for it, if we define
\[(e_{[i,j]})_k:= \frac1{\sqrt{j-i+1}}\begin{cases}1,\, \text{ if } k\in[i,j]\\ 0,\,\,\text{else}\end{cases}.\]
As we can align all elements of $J = \{j_1,j_2,\ldots, j_s\}$ with $1\leq j_1<j_2<\ldots < j_s =n$, we see that $\{e_{[1,j_1]},e_{[j_1+1,j_2]},e_{[j_2+1,j_3]},\ldots,e_{[j_{s-1}+1,j_s]}\}$ forms an ONB of $K_J$.
Now, we can write all elements $x\in K_J\cap B_2^n$ as $x = \sum_{i=1}^s \alpha_i e_{[j_{i-1}+1,j_i]}$ by setting $j_0:=0$. The property that $x\in B_2^n$ now enforces (ONB) that $\Vert \alpha \Vert_2\leq 1$.  Now, note that $K_0^s = -K_0^s$, so we have 
\[w(K_0^s) = \Ex \sup_{x\in K_0^s-K_0^s}\ip{g}{x} = 2\Ex \sup_{x\in K_0^s}\ip{g}{x}.\]

Using the decomposition $K_0^s = \bigcup_{|J| = s}\left(K_J\cap B_2^n\right)$, we get
\[w(K_0^s)  =  2\Ex \sup_{|J|= s}\sup_{x\in K_J\cap B_2^n}\ip{g}{x}.\]
Now 
\[\sup_{x\in K_J\cap B_2^n}\ip{g}{x} \leq \sup_{\alpha\in B_2^s}\sum_{i=1}^s \alpha_i\ip{g}{e_{[j_{i-1}+1,j_i]}}= \sup_{\alpha\in B_2^s}\sum_{i=1}^s \alpha_i\underbrace{\sum_{k = j_{i-1}+1}^{j_i} \frac{g_k}{\sqrt{j_i-j_{i-1}}}}_{=:G_i^J}.\]
Note that $G_i^J$ is again a Gaussian random variable with mean $0$ and variance $1$. Furthermore, the supremum over $\alpha$ is attained, if $\alpha$ is parallel to $G^J$, so we have
$\sup_{x\in K_J\cap B_2^n}\ip{g}{x} = \Vert G^J\Vert_2$. Also note that $G^J$ has i.i.d. entries, but for different $J_1,J_2$, the random vectors $G^{J_1}$ and $G^{J_2}$ may be dependent.
Our task is now to calculate $\Ex\sup_{|J|=s}\Vert G^J\Vert_2$.
As it has been shown for example in~\cite{foucart2013mathematical}, we have that
\[\sqrt{\frac2\pi}\sqrt{s}\leq \Ex\Vert G^J\Vert_2\leq \sqrt{s}\]
and from standard results for Gaussian concentration (cf.~\cite{plan2013robust}), we get
\[\Prob(\Vert G^J\Vert_2\geq\sqrt{s} + t)\leq \Prob(\Vert G^J\Vert_2\geq\Ex\Vert G_J\Vert_2 + t)\leq \ee^{-t^2/2}.\]
By noting that $|\{J\subset[n]\colon |J|=s\}| = { n\choose s}$, we see by a union bound that

\[
\Prob(\sup_{|J|=s}\Vert G^J\Vert_2\geq\sqrt{s} + t) \leq {n\choose s}\Prob(\Vert G^J\Vert_2\geq\sqrt{s} + t)\leq {n\choose s}\ee^{-t^2/2}.
\]

For the following calculation, set $X:= \sup_{|J|=s}\Vert G^J\Vert_2$. By Jensen's inequality and rewriting the expectation, we have that
\[\ee^{\lambda \Ex X}\leq \Ex \ee^{\lambda X} = \int_0^\infty \Prob(\ee^{\lambda X}\geq \tau)\dx \tau.\]
Now, the previous consideration showed, that 
\[\Prob(\ee^{\lambda X}\geq\underbrace{\ee^{\lambda (\sqrt{s} + t)}}_{=:\tau}) = \Prob(X\geq\sqrt{s} + t)\leq  {n\choose s}\ee^{-t^2/2}=  {n\choose s}\ee^{-(\log(\tau)/\lambda -\sqrt{s})^2/2},
\]
Computing the resulting integrals yields 
\begin{equation*}
\ee^{\lambda \Ex X}\leq{n\choose s} \ee^{-s/2}\lambda\sqrt{2\pi}\ee^{(\sqrt{s}+\lambda)^2/2}.
\end{equation*}

Using a standard bound for the binomial coefficients, namely ${n\choose s}\leq \ee^{s \log (\ee n/s)}$, we see

\[\ee^{\lambda \Ex X}\leq \ee^{s\log(\ee n/s) - s/2 +(\sqrt{s} + \lambda)^2/2+\log(\lambda)+\log(\sqrt{2\pi})},\]
or equivalently
\[\lambda \Ex X \leq s\log(\ee n/s) - s/2 +(\sqrt{s} + \lambda)^2/2+\log(\lambda)+\log(\sqrt{2\pi})\]
By setting $\lambda = \sqrt{s\log(\ee n/s) }$ and assuming (reasonably) large $n$, we thus get
\[\Ex X\leq 5 \sqrt{s\log(\ee n/s) }.\]
From this, we see that
\[w(K_0^s)\leq 10\sqrt{s\log(\ee n/s) }.\]

It follows that the Gaussian mean width of the set of gradient sparse vectors is the same as the mean width of sparse vectors due to the similar structure.
If we want to obtain accuracy $\delta$ for our reconstruction, according to Theorem~\ref{theo:feasibility}, we need to take
\[m = \Ocal\left(\frac{s\log(\ee n/s)}{\delta^2}\right)\] 
measurements.

In Compressed Sensing, the squared mean width of the set of $s$-sparse vectors (its so called \emph{statistical dimension}) already determines the number of required measurements in order to recover a sparse signal with basis pursuit. This is the case because the convex hull of the set of sparse vectors can be embedded into the $\ell_1$-ball inflated by a constant factor.
In the case of TV minimization, as we will see in the following section, this embedding yields a (rather large) constant depending on the dimension.
 
\subsection{The extension to gradient compressible vectors needs a new approach}

In the previous subsection, we considered exactly gradient sparse vectors. However searching all such vectors $x$ that satisfy $Ax=y$ is certainly not a feasible task. Instead, we want to solve the convex program

\[\min\Vert z\Vert_{TV} \,\text{ with } Az = y,\]
with $\Vert z\Vert_{TV} = \Vert \nabla z\Vert_1$ the total variation seminorm. Now if we have that $x\in K_0^s$, we get that
\[\Vert x\Vert_{TV}  \leq 2\Vert \alpha\Vert_1 \leq 2\sqrt{s}\Vert\alpha\Vert_2 = 2\sqrt{s},\]
with $\alpha$ as in section~\ref{sec:GradSparse}, so $K_0^s\subset K_{TV}^{2\sqrt{s}}:=\{x\in B_2^n\colon \Vert x\Vert_{TV}\leq 2\sqrt{s}\}$. As $K_{TV}^{2\sqrt{s}}$ is convex, we even have $\ch(K_0^s)\subset K_{TV}^{2\sqrt{s}}$.
We can think of the set $K_{TV}^{2\sqrt{s}}$ as 'gradient- compressible' vectors.

In the proof of Theorem 3.3 in~\cite{cai2015guarantees}, the Gaussian width of the set $K_{TV}^{4\sqrt{s}}$ has been calculated via a wavelet-based argument. One obtains that $w(\Ktv)\leq C\sqrt{\sqrt{ns}\log(2n})$ with $C\leq20$ being an absolute constant. In this section we illustrate, that proof techniques different from the ones used in the case of synthesis sparsity are indeed necessary in order to obtain useful results. In the synthesis case, the $1$-norm ball of radius $\sqrt s$ is contained in the set of $s$-sparse vectors inflated by a constant factor. This in turn implies that the mean width of the compressible vectors is bounded by a constant times the mean width of the $s$-sparse vectors.

We will attempt a similar computation, that is to find a constant, such that the set $K_{TV}^{2\sqrt{s}}$ is contained in the 'inflated' set $c_{n,s} \ch(K_0^s)$. Then $w(\Ktv)\leq c_{n,s} w(K_0^s)$. Although this technique works well for sparse recovery, where $c_{n,s} = 2$, it pityably fails in the case of TV recovery as we will see below.

Let us start with $x\in \Ktv$. Now we can decompose $J:=\tvsupp(x) = J_1\uplus J_2\uplus\ldots J_p$ with $|J_k|\leq s$ in an ascending manner, i.e., for all $k\in J_i, l\in J_{i+1}$, we have that $\alpha_k<\alpha_l$. Note that the number $p$ of such sets satisfies $p\leq \frac{n}{s}$.
Similarly as above, we now write $x = \sum_{i=1}^{|J|}\alpha_i e_{[j_{i-1}+1,j_i]} = \sum_{k=1}^p\sum_{i\in J_k}\alpha_i e_{[j_{i-1}+1,j_i]}$. From this, we see that 
\[x =  \sum_{k = 1}^p \Vert \alpha_{J_k}\Vert_2 \underbrace{\sum_{i\in J_k}\frac{\alpha_i}{\Vert \alpha_{J_k}\Vert_2} e_{[j_{i-1}+1,j_i]}}_{\in K_0^s}.\]
The necessary factor $c_{n,s}$ can be found by bounding the size of $\Vert \alpha_{J_k}\Vert_2$, namely
\[\max (\Vert \alpha_{J_k}\Vert_2)\leq \sum_{k=1}^p\Vert \alpha_{J_k}\Vert_2\stackrel{C-S}{\leq} \underbrace{\Vert \alpha\Vert_2}_{\leq 1} \sqrt{p}\leq\sqrt{\frac{n}{s}}.\]

From this, we see that $\Ktv\subset \sqrt{\frac{n}{s}} \ch(K_0^s)$. To see that this embedding constant is optimal, we construct a vector, for which it is needed.

To simplify the discussion, suppose that $n$ and $s$ are even and $s|n$. 
%The vector $x_1 = (\sqrt{\frac{1+\varepsilon}{n}},\sqrt{\frac{1-\varepsilon}{n}},\sqrt{\frac{1+\varepsilon}{n}},\sqrt{\frac{1-\varepsilon}{n}},\ldots)$ (consider even $n$) has 2-norm $1$, lies in $\Ktv$ for $\varepsilon<\frac{2\sqrt{s}}{n}$ and has jump support on all of $[n]$!
For even $n$, the vector $x_1 = (\sqrt{\frac{1-(-1)^k\varepsilon}{n}})_k$ has unity norm, lies in $\Ktv$ for $\varepsilon<\frac{2\sqrt{s}}{n}$ and has jump support on all of $[n]$!

For a vector $x\in \R^n$ and an index set $I\subset [n]$, we define the restriction of $x$ to $I$ by \[(x|_I)_j :=\begin{cases}x_j\text{, if }j\in I\\
0\text{, else}.\end{cases}\]
By splitting $\tvsupp(x_1)$ into sets $J_1,\ldots,J_{n/s}$ and setting $a_k = \sqrt{\frac ns}x_1|_{J_k}\in K_0^s$, we see that $x_1= \sum_{k=1}^{n/s} \sqrt{\frac sn} a_k$ and in order for this to be elements of $c_{n,s}\ch(K_0^s)$, we have to set $c_{n,s} = \sqrt{\frac ns}$. This follows from
\[x_1= \sum_{k=1}^{n/s} x_1|_{J_k}=\sum_{k=1}^{n/s} \sqrt{\frac sn} \frac{p}{p}a_k =  \sum_{k=1}^{n/s} \frac{1}{p} \underbrace{\left(\sqrt{\frac ns}a_k\right)}_{\in \sqrt{\frac ns} K_0^s}\in \sqrt{\frac ns}\ch(K_0^s)\]
and no smaller inflation factor than $\sqrt{\frac ns}$ can suffice.\\

So from the previous discussion, we get
{\lemma\label{lemma:inclusions} We have the series of inclusions
	\[\ch(K_0^s)\subset \Ktv \subset \sqrt{\frac ns}\ch(K_0^s).\]}

In view of the results obtainable for sparse vectors and the $\ell_1$-ball, this is very disappointing, because Lemma~\ref{lemma:inclusions} now implies that the width of $\Ktv$ satisfies 
\[w(\Ktv)\leq w\left(\sqrt{\frac ns}\ch(K_0^s)\right) = \sqrt{\frac ns} w(K_0^s)\leq 10\sqrt{n\log(\ee (n-1)/s)},\]
which is highly suboptimal. 

Luckily, the results in~\cite{cai2015guarantees} suggest, that the factor $n$ in the previous equation can be replaced by $\sqrt{sn}$. However, they have to resort to a direct calculation of the Gaussian width of $\Ktv$. The intuition why the Gaussian mean width can be significantly smaller than the bound given in Lemma~\ref{lemma:inclusions} stems from the fact, that in order to obtain an inclusion we need to capure all 'outliers' of the set - no matter how small their measure is.


\subsection{Exact recovery}\label{sec:ExactRecov}

 For exact recovery, the $M^*$-bound is not suitable anymore and, as suggested in~\cite{vershynin2014estimation}, we will use 'Gordon's escape through the mesh' in order to find conditions on exact recovery. Exact recovery for TV minimization via this approach has first been considered in~\cite{cai2015guarantees}. 

%We will connect their approach via the TV-null space property to our approach in this section.

Suppose, we want to recover $x\in K_0^s$ from Gaussian measurements $Ax =y$. Given, that we want our estimator $\hat x$ to lie in a set $K$, exact recovery is achieved, if $K\cap \{z\colon Az = y\} = \{x\}$. This is equivalent to requiring
\[(K-x)\cap  \underbrace{\{z-x \colon Az = y\}}_{=\ker(A)}  = \{0\}.\]
With the descent cone $D(K,x) = \{t(z-x)\colon t\geq0,z\in K\}$, we can rewrite this condition as 
\[D(K,x)\cap  \ker(A) = \{0\},\]
by introducing the set $S(K,x) = D(K,x)\cap B_2^n$, we see that if
\[S(K,x)\cap  \ker(A) =\emptyset,\]
we get exact recovery.
The question, when a section of a subset of the sphere with a random hyperplane is empty is answered by Gordon's escape through a mesh.
{\theo[\cite{gordon1988milman}] Let $S\subset \S^{n-1}$ be fixed and $E\in G_{n,n-m}$ be drawn at random according to the Haar measure. Assume that $\hat w(S)=\Ex \sup_{u\in S}\ip{g}{u}<\sqrt{m}$, then $S\cap E=\emptyset$ with probability exceeding 
	\[1-2.5\exp\left(-\frac{(m/\sqrt{m+1}-\hat w(S))^2}{18}\right).\]
}

So we get exact recovery with high probability from a program given in Theorem~\ref{theo:feasibility} or~\ref{theo:opti}, provided that $m>\hat w(S(K,x_0))^2$.

Let's see how this applies to TV minimization. Suppose, we are given $x\in K_0^s$ and Gaussian measurements $Ax=y$. Solving
\[\min\Vert z\Vert_{TV} \,\text{ with } Az = y,\]
amounts to using the Minkowski functional of the set $K = \{z\in\R^n\colon \Vert z\Vert_{TV}\leq \Vert x\Vert_{TV}\}$, which is a scaled TV-Ball.

In~\cite{cai2015guarantees}, the null space property for TV minimization given in Corollary~\ref{corr:TVNSP} has been used in order to obtain recovery guarantees.

They consider the set, where this condition is not met
\[\Scal := \{x'\in B_2^n\colon \exists J \subset[n],|J|\leq s, \Vert(\nabla x')_J\Vert_1 \geq \Vert (\nabla x')_{J^c}\Vert_1\},\]
and apply Gordon's escape through the mesh to see that with high probability, its intersection with the kernel of $A$ is empty, thus proving exact recovery with high probability. Their estimate to the mean width of the set $\Scal$, 
\[\hat w(\Scal)\leq c \sqrt[4]{ns}\sqrt{\log(2n)}\]
with $c<19$ is essentially optimal (up to logarithmic factors), as they also show that $w(\Scal)\geq C \sqrt[4]{ns}$.
So uniform exact recovery can only be expected for $m =\Ocal(\sqrt{sn}\log n)$ measurements.

Let us examine some connections to the previous discussion about the descent cone.

{\lemma We have that for $K = \{z\in\R^n\colon \Vert z\Vert_{TV}\leq \Vert x\Vert_{TV}\}$ defined as above and $x\in K_0^s$, it holds that $S(K,x)\subset \Scal$.
}
\begin{proof}
	Let $y\in S(K,x)$. Then there exists a $x\neq z\in K$, such that $y = \frac{z-x}{\Vert z-x\Vert_2}$. Set $J=\tvsupp(x)$, then, as $z\in K$, we have that $\Vert z\Vert_{TV}\leq \Vert x\Vert_{TV}$, or
	\[\sum_{i\in J} |(\nabla x)_i|\geq \sum_{i\in J} |(\nabla z)_i|+\sum_{i\not\in J} |(\nabla z)_i|\]
	Now, by the triangle inequality and this observation, we have
	\[\sum_{i\in J} |(\nabla x)_i- (\nabla z)_i|\geq \sum_{i\in J} |(\nabla x)_i|- |(\nabla z)_i|\geq \sum_{i\not\in J} |(\nabla z)_i| = \sum_{i\not\in J} |(\nabla x)_i- (\nabla z)_i|.\]
	The last equality follows from the fact that $\nabla x$ is zero outside of the gradient support of $x$. Multiplying both sides with $\frac1{\Vert z-x\Vert_2}$ gives the desired result
	\[\Vert(\nabla y)_J\Vert_1 =\frac1{\Vert z-x\Vert_2} \sum_{i\in J} |(\nabla x)_i- (\nabla z)_i|\geq\\ \geq\frac1{\Vert z-x\Vert_2} \sum_{i\not\in J} |(\nabla x)_i- (\nabla z)_i|=\Vert(\nabla y)_{J^c}\Vert_1. \]
	
\end{proof}

The previous lemma shows that the recovery guarantees derived from the null space property and via the descent cone are actually connected in a very simple way.


Clearly, now if we do not intersect the set $\Scal$, we also do not intersect the set $S(K,x)$, which yields exact recovery for example with the same upper bounds on $m$ as for $\Scal$. 
Even more specifically, in the calculation of $\hat w(\Scal)$ given in~\cite{cai2015guarantees}, an embedding into a slightly larger set $\tilde \Scal = \{x\in B_2^n\colon \Vert x\Vert_{TV}\leq 4\sqrt{s}\}$ is made. This embedding can also quite easily be done if we note that $\Vert x\Vert_{TV}\leq 2\sqrt{s}$, as we showed above and $\Vert z\Vert_{TV}\leq \Vert x\Vert_{TV}$.

Note that the same discussion also holds for higher dimensional signals, such that the improved numbers of measurements as given in Section~\ref{sec:RecoveryGauss} can be applied.

\subsection{Subgaussian measurements}\label{subsec:Subgaussian}

Up to this point, all our measurement matrices have been assumed to consist of i.i.d.~Gaussian random variables. We will reduce this requirement in this section to be able to incorporate also subgaussian measurement matrices into our framework. 

\begin{defi}\label{defi:subgauss}
	A real valued random variable $X$ is called \emph{subgaussian}, if there exists a number $t>0$, such that $\Ex \ee^{tX^2}<\infty$.
	A real valued random vector is called subgaussian, if all of its one dimensional marginals are subgaussian.
\end{defi}
An obvious example of subgaussian random variables are Gaussian random variables, as the expectation in Definition~\ref{defi:subgauss} exists for all $t<1$. Also, all bounded random variables are subgaussian.

Here, we rely on results given by Tropp in~\cite{tropp2014convex} using the results of Mendelson~\cite{koltchinskii2015bounding, mendelson2014learning}.
We will consider problems of the form
\begin{equation}\label{eq:minNoise}
\min \Vert z\Vert_{TV}\,\text{ such that } \Vert Az - y\Vert \leq\varepsilon,
\end{equation}
where $A$ is supposed to be a matrix with independent subgaussian rows. Furthermore, we denote the exact solution by $x_0$, i.e., $Ax_0 = y$.
We pose the following assumptions on the distribution of the rows of $A$. 
\begin{enumerate}
	\item[(M1)] $\Ex A_i = 0$,
	\item[(M2)] There exists $\alpha>0$, such that for all $u\in\S^{n-1}$ it holds that $\Ex|\langle A_i,u\rangle|\geq\alpha$,
	\item[(M3)] There is a $\sigma>0$, such that for all $u\in\S^{n-1}$ it holds that $\Prob(|\langle A_i,u\rangle|\geq t)\leq2\exp(-t^2/(2\sigma^2))$,
	\item[(M4)] The constant $\rho:= \frac\sigma\alpha$ is small.
\end{enumerate}

Then the small ball methods yields the following recovery guarantee (we present the version of \cite{tropp2014convex}).
{\theo\label{thm:TroppRecovery} Let $x_0\in\R^n$ and $A\in\R^{m\times n}$ be a subgaussian matrix satisfying (M1)-(M4) above. Furthermore, set $y = Ax_0+e$, where $\Vert e\Vert\leq \varepsilon$ denotes the (bounded) error of the measurement.
	Then the solution $\hat x$ of~\eqref{eq:minNoise} satisfies 
	\[\Vert \hat x - x_0\Vert \leq \frac{2\varepsilon}{\max\{c\alpha\rho^{-2}\sqrt{m} - C\sigma w(S(K,x_0))-\alpha t,0\}}\]
	with probability exceeding $1-\ee^{-ct^2}$. $D(K,x_0)$ denotes the descent cone of the set $K$ at $x_0$, as defined in the previous section.}


From this we see that, provided \[m\geq \tilde C\rho^6 w^2(S(K,x_0)),\] we obtain stable reconstruction of our original vector from~\eqref{eq:minNoise}. 
Note that the theorem is only meaningful for $t=\Ocal(\sqrt{m})$, as otherwise the denominator vanishes.

In the previous section, we have shown the inclusion $S(K,x_0)\subset \Scal$ for $x_0\in K_s^0$ and hence we have that 
\[w(S(K,x_0)\leq w(\Scal)\leq c \sqrt[4]{ns}\sqrt{\log(2n)}.\]

So we see that for $m\geq \tilde C\rho^6 \sqrt{ns}\log(2n)$, we obtain the bound

\begin{align*}\Vert \hat x - x_0\Vert &\leq \frac{2\varepsilon}{\max\{c\alpha\rho^{-2}\sqrt{\tilde C} \rho^3  \sqrt[4]{ns}\sqrt{\log(2n)} - C\sigma \sqrt[4]{ns}\sqrt{\log(2n)}-\alpha t,0\}}\\
& = \frac{2\varepsilon}{\max\{\sigma(c\sqrt{\tilde C} - C) \sqrt[4]{ns}\sqrt{\log(2n)}-\alpha t,0\}}
\end{align*} 

with high probability. We conclude that, given the absolute constants $c,C$, we need to set $\tilde C\geq \tfrac{C^2}{c^2}$ in order to obtain a meaningful result. Combining all our previous discussions with Theorem~\ref{thm:TroppRecovery}, we get

\begin{theo}\label{theo:SubgaussGuarantee}
	Let $x_0\in\R^n$, $m\geq \tilde C\rho^6 \sqrt{ns}\log(2n)$ and $A\in\R^{m\times n}$ be a subgaussian matrix satisfying (M1)-(M4). Furthermore, set $y = Ax_0+e$, where $\Vert e\Vert\leq \varepsilon$ denotes the (bounded) error of the measurement, constants $c,C,\tilde C>0$ as above and $t\leq \frac{\sigma(c\sqrt{\tilde C} - C) \sqrt[4]{ns}\sqrt{\log(2n)}}{\alpha}$.
	Then the solution $\hat x$ of~\eqref{eq:minNoise} satisfies 
	\[\Prob\left(\|\hat x - x_0\| > \frac{2\eps}{\sigma(c\sqrt{\tilde C} - C) \sqrt[4]{ns}\sqrt{\log(2n)}-\alpha t}\right)\leq \ee^{-ct^2}. \]
\end{theo}

We can for example set $t = \rho (c\sqrt{\tilde C} -C) \sqrt[4]{ns}$ (for $n\geq 2$) to obtain the bound

\[\Prob\left(\|\hat x - x_0\| > \frac{2\eps}{\sigma(c\sqrt{\tilde C} - C) \sqrt[4]{ns}(\sqrt{\log(2n)}-1)}\right)\leq \ee^{-\tilde c \rho \sqrt{ns}}.\]

For example for i.i.d. standard Gaussian measurements, the constant $\rho = \sqrt{\frac2\pi}$.

Note that in the case of noisefree measurements $\eps = 0$, Theorem~\ref{theo:SubgaussGuarantee} gives an exact recovery result for a wider class of measurement ensembles with high probability. Furthermore with a detailed computation of $w(S(K,x_0))$ one may be able to improve the number of measurements for nonuniform recovery. It also remains open, whether the lower bounds of Cai and Xu for the case of Gaussian measurements can be generalized to the subgaussian case. In fact, our numerical experiments summarized in Figure~\ref{fig:Phase} suggest a better scaling in the ambient dimension, around $N^{1/4}$, in the average case. We consider it an interesting problem for future work to explore whether this is due to a difference between Rademacher and Gaussian matrix entries, between uniform and nonuniform recovery, or between the average and the worst case. Also, it is not clear whether the scaling is in fact $N^{1/4}$ or if the observed slope is just a linearization of, say, a logarithmic dependence.


\begin{figure}
	\centering
	\includegraphics[width= 0.45\textwidth]{LogscalePhaseTrans.pdf}\quad
	\includegraphics[width= 0.47\textwidth]{LogscalePhaseTransLogAxis.pdf}
	\caption{Average error of recovery from Rademacher measurements in $1d$ with $m$ measurements and ambient dimension $N$ for fixed cosparsity level $s = 5$. Left: linear axis scaling, Right: logarithmic axis scaling. The slope of the phase transition in the log-log plot is observed to be about $\frac14$.}
	\label{fig:Phase}
\end{figure}
